MAP: Multi-user Personalization with Collaborative LLM-powered Agents

The widespread adoption of Large Language Models (LLMs) and LLM-powered agents in multi-user settings underscores the need for reliable, usable methods to accommodate diverse preferences and resolve conflicting directives. Drawing on conflict resolution theory, we introduce a user-centered workflow for multi-user personalization comprising three stages: Reflection, Analysis, and Feedback. We then present MAP -- a \textbf{M}ulti-\textbf{A}gent system for multi-user \textbf{P}ersonalization -- to operationalize this workflow. By delegating subtasks to specialized agents, MAP (1) retrieves and reflects on relevant user information, while enhancing reliability through agent-to-agent interactions, (2) provides detailed analysis for improved transparency and usability, and (3) integrates user feedback to iteratively refine results. Our user study findings (n=12) highlight MAP's effectiveness and usability for conflict resolution while emphasizing the importance of user involvement in resolution verification and failure management. This work highlights the potential of multi-agent systems to implement user-centered, multi-user personalization workflows and concludes by offering insights for personalization in multi-user contexts.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
 
\subsection{Generalizable Insights for User-centered LLM-based Agent Systems}
There is growing interest in developing LLM-based agents and orchestrating them to tackle complex tasks~\cite{xi2023agentsurvey, hong2024metagpt}. Our work underscores that, for these systems to be usable and widely accepted by users, it is crucial to first develop a clear workflow and design principles, and then construct the LLM-powered agent system to support this framework. We present the first framework for collaborative LLM-powered agents in the context of multi-user personalization, providing a reference model for developing usable, collaborative LLM-based agents beyond this specific scope.

Our approach begins by identifying the unique and complex dynamics inherent in multi-user environments, where conflicting preferences and needs frequently arise. These conflicts necessitate strategies that can merge, negotiate, and adapt to a diverse range of preferences. Recognizing the increasing deployment of AI systems in such settings, we propose a workflow that supports three critical stages: reflection, analysis, and feedback, with specific agents assigned to handle these functionalities.

For the reflection stage, we employ an agent with RAG (\ie Document Handler) to efficiently retrieve relevant user rules and preferences from documents. Without this component, a monolithic, simple LLM-based agent would struggle to provide a functional reflection stage. Users would be forced to manually track and input all rules for every interaction to ensure the system is aware of them. In contrast, with our system, each user only needs to maintain their own set of rules, which the Document Handler agent accesses to keep up-to-date, retrieving relevant information as needed. This process is further supported by the Rule Manager agent, which monitors the retrieval results to enhance performance.

For the analysis and feedback stages, we assign a dedicated agent (\ie Planner) to focus solely on these tasks, allowing the Document Handler and Rule Manager to manage the reflection stage. Our user study findings (Section~\ref{sec:user-study-findings}) reveal that the analysis and feedback stages are crucial for user engagement and system adaptability, but often involve digesting complex information, understanding nuances that may lead to conflicts, and generating adapted solutions.
A dedicated Planner agent, rather than a monolithic agent handling everything, ensures a smoother workflow, improves conflict resolution performance (Figure~\ref{fig:eval}), and enhances overall system efficiency.


\subsection{Flexible Extension of the System with Newly Emerging User Needs}
Deploying the system in real-world settings provides invaluable insights into its limitations and reveals emerging user needs.
As demonstrated in our user study, users expressed a strong demand for greater control, verification tools, and more robust mechanisms to handle conflict resolution failures. For example, participants emphasized the need for more customizable outputs, quick-action interfaces, and deterministic verification tools to ensure accuracy and prevent errors in high-stakes scenarios.

% Our approach—understanding the task and desired workflow, and then breaking down the ultimate task into manageable steps—becomes even more effective as we scale to more complex, real-world multi-user personalization scenarios.
% This modular design allows for explicit specification of subtasks, enhancing both flexibility and scalability.
Our modular approach—using a system of orchestrated submodules, each represented by LLM-based agents—proves highly beneficial in meeting these needs. The flexibility of our design allows for explicit specification of subtasks and components within a complex task. As new needs emerge, such as enhanced user control, verification steps, or improved conflict resolution, our modular system can be extended accordingly. For instance, based on user feedback, we could introduce a \textit{critic} agent~\cite{madaan2024selfcritic, choi2024malade} paired with the Planner agent to iteratively verify the Planner's output, further improving the system's reliability and user satisfaction.
Additionally, beyond relying solely on non-deterministic LLMs, our modular design also supports integrating deterministic programs to improve reliability for well-defined tasks~\cite{choi2024malade}. For instance, deterministic function calls can be used for verification and failure control in rule retrieval, ensuring that the system performs consistently and accurately. This combination of LLMs and deterministic components offers a more robust framework for handling complex scenarios.

Overall, our modular approach allows for the incremental addition of new agents or components, can effectively address evolving user needs, and maintain system usability.
This is not only advantageous for multi-user personalization but can also be generalized to the construction of collaborative LLM-powered agents for a wide range of complex, user-centered tasks.




%\subsection{Implications}
\subsection{Enhancing Multi-User Personalization with Verification Methods}
Our findings highlight a critical need for verification methods and tools to accompany multi-user personalization workflows. In multi-user settings, participants found it difficult to track others' rules, assess adherence to those rules, and detect conflicts. When the system made errors in rule retrieval or rule adherence during conflict resolution, users struggled to detect or address these failures. This complexity led users to often accept the system's suggestions blindly, as managing multiple users’ needs was seen as a time-consuming and challenging task. The lack of awareness of system failures negatively impacted user reliance, usability, and satisfaction, emphasizing the need for verification tools like explanations. The issue of lack of verification methods became more severe in high-stakes environments, such as our hospital simulation, where users noted that the consequences of undetected failures could be dire. As a result, participants advocated for stronger verification mechanisms, such as preemptive failure analysis before plans were delivered to users.

To meet these needs, different verification approaches can be integrated into our multi-user personalization workflow to enhance reliability and usability. Explanations can be designed to help users understand which rules were missed or where uncertainty exists \cite{slack2021reliable}, supporting system transparency and enabling users to allocate their attention effectively. Additionally, more rigorous verification mechanisms, such as formal verification techniques like model checking \cite{baier2008principles}, can be employed to ensure that essential rules are strictly enforced in the generated plans. The integration of formal techniques with our multi-user personalization workflow can ensure that only plans adhering to all relevant and specified constraints are presented to the user, making it more reliable and usable for high-stakes settings. Future implementations should explore different verification methods based on the severity of the risk and the diverse needs of the deployment context and users.

% Our findings suggest that through using our multi-user personalization workflow and \oursend, LLMs can provide users with personalization on two distinct levels: individually within a group, and across the broader group setting. At the individual level, personalization is facilitated by allowing users to receive tailored outputs that specifically align with their unique preferences or requests even when there are many other considerations (\eg conflict with other users' needs). Such personalization can be provided to multiple users simultaneously, as the AI system identifies, resolves, or seeks feedback to resolve conflicts between preferences. Furthermore, AI systems communicate such changes or related updates to different users and obtain additional feedback if needed, ensuring that the needs of multiple users are met and coexist harmoniously within the group's ecosystem.

% On the group level, the multi-user personalization workflow allows AI systems to adapt to diverse needs across various deployment contexts. Through the MAP framework, it becomes possible for users to adjust their preference list to encapsulate the group's preferences, values, norms, and context-specific demands. Leveraging this information, AI systems can predict a group's preferred approach to resolving unforeseen issues, such as devising a solution that aligns with the preferences of the majority of the group's users. Additionally, the level of user involvement preferred for such situations can be derived by the AI system storing the group's usual patterns of interaction in its database. Based on these tailored inputs, AI systems can devise and execute strategies that align with the group's objectives and the prevailing environment.

% The existing research on LLMs highlights how AI-powered agents can gather and interpret human preferences collectively and mimic human behaviors \cite{ma2023beyond, papachristou2023leveraging, bakker2022fine}. These advances provide great opportunities to explore how to leverage these technologies to develop AI systems that are useful in practical settings where both individual and group dynamics exist. Our study contributes towards addressing these considerations.



% \jihye{@self:add discussion on improving the RAG pipeline for more complicated tasks with larger-sized documents, etc. dynamically loading only relevant rules not to be limited by context length}

\section{Limitations and Future Work}
Our work has several limitations. First, while we designed scenarios based on three use cases—assistive care, households, and workplaces—there are broader and more complex scenarios that could be applied to our multi-user personalization framework. Although our study does not cover highly complex tasks, it demonstrates the potential application of our system in this space, which can be expanded in future work by testing the workflow in more complex settings to assess usability and effectiveness.
Second, we lack an exhaustive technical evaluation measuring the performance of our system. As our focus was on the benefits of incorporating a multi-agent structure to realize the multi-user personalization workflow, our performance comparisons were limited to comparisons with the most basic single LLM-based chat agent. Future research could explore alternative technical approaches and evaluate system performance and reliability.
Third, our robot study was conducted on a small scale with a limited number of participants. Since the goal was to demonstrate a practical application, the study used a simulation rather than a full-scale implementation in a hospital setting. Future work could expand this opportunity to explore the system’s practical application in real-world environments. Finally, the exploratory and qualitative nature of our study restricts the generalizability of our findings. Future studies could use more exhaustive and quantitative methods with larger datasets to validate or enhance our results.

==> figure_quant.tex <==
\begin{figure}[t]
\centering
  \includegraphics[height=2.6in]{figures/quant.pdf}
%   \vspace{-12pt}
  \caption{\textit{Quantitative Data} --- Data points on user usability, satisfaction, ease of use, and ease of learning measured during the user study. Horizontal lines indicate significant pairwise comparisons with a paired t-test ($p < 0.05^{\ast}$, $p < 0.01^{\ast\ast}$, $p < 0.001^{\ast\ast\ast}$). }
  \label{fig:quant}
%   \vspace{-6pt}
\end{figure}



==> figure_teaser.tex <==
\begin{figure*}[!th]
  \includegraphics[width=\textwidth]{figures/teaser new.pdf}
   \vspace{-12pt}
  \caption{\textit{Outline of the MAP framework and \ours ---} In this paper, we draw from lifelong learning theories of the education domain to design a framework that supports AI systems in providing personalization to multiple users across three stages: \textit{reflection}, \textit{articulation}, and \textit{feedback}. We implement our framework using multiple LLM agents that operate within a hierarchical structure, employing retrieval-augmented generation techniques.
}
  \label{fig:teaser}
%   \vspace{-6pt}
\end{figure*}



==> implementation.tex <==
% \section{MAPS Implementation: RAG-based LLM}
% \subsection{Implementation Details}
\section{\oursend: Our System for Multi-user Personalization}
\label{sec:system}
To operationalize our multi-user personalization workflow, we implemented an integrated system.
In this section, we present the implementation of our multi-user personalization workflow, called \oursend. Our implementation leverages the orchestration of three LLM-based agents: Document Handler with Retrieval Augmented Generation (RAG), Rule Manager, and Planner. They collaborate with each other with the purpose of supporting the three stages of the multi-user personalization workflow introduced in Section~\ref{sec:workflow}: reflection, articulation, and feedback.
In Section~\ref{sec:ours-primitives}, we delineate design primitives of a generic LLM-based agent: an agent that encapsulates an LLM along with tool usage and memory integration.
Subsequently, leveraging these primitives, we delve into the actual implementation of our agents and their orchestration in Section~\ref{sec:ours-details}.



%In this section, we present our Retrieval Augmented Generation (RAG) approach, namely \oursend, which serves as the instantiation of the MAP framework detailed in Section~\ref{sec:fw2}. 
% Initially, we delineate the primitives of LLM-powered agents and their orchestration in Section~\ref{sec:ours-primitives}. 
%\ours leverages the hierarchical orchestration of three LLM-based agents: Rule Manager, Document Handler, and Planner. They collaborate with each other with the purpose of supporting the three stages of the MAP framework introduced in Section~\ref{sec:fw2}: reflection, articulation, and feedback.
%In Section~\ref{sec:ours-primitives}, we delineate design primitives of a generic LLM-based agent: an agent that encapsulates an LLM along with tool usage and memory integration.
%Subsequently, leveraging these primitives, we delve into the actual implementation of our agents and their orchestration in Section~\ref{sec:ours-details}.

% \subsection{Design Primitives}
\subsection{Preliminaries: Design Primitives of LLM-based Agents}
\label{sec:ours-primitives}
% Given the remarkable abilities of LLMs, a pivotal question arises: how can we best harness their power to tackle complex tasks?
While today's LLMs exhibit impressive capabilities, they remain constrained by technical and practical limitations such as brittleness, non-determinism, limited context window, inference costs, and latency~\cite{liang2023holistic, xie2021explanation}. In other words, one cannot simply give high-level instructions to an LLM and expect it to accomplish a task, with these limitations becoming more pronounced as the complexity of the target task or application increases. 
Consequently, to best harness the capability of an LLM as a component of a complicated task, it is necessary to decompose the task into sub-tasks and manage multiple LLM conversations, each equipped with its own set of specifically-defined instructions, state, and data sources.

% When attempting to build a non-trivial application, one inevitably encounters the necessity to decompose a task into sub-tasks and manage multiple LLM conversations, each with its own set of instructions, state, and data sources.

%\textbf{Agent.}
\paragraph{Agent}
A natural and convenient abstraction for managing such complexity is the notion of an agent who is instructed to be responsible for a specific aspect of the task.
An agent is essentially an ``intelligent'' entity that can respond to, and transform messages.
% ,  \ie an agent is a \textit{message transformer}.
Typically, an agent encapsulates an LLM (\eg an interface to GPT-4 in our implementation) and may also be equipped with so-called \textit{tools} (also known as functions or plugins) and \textit{memory} such as conversation history or a vector database (described below).  
Much like a team of humans, agents interact by exchanging messages.
And importantly, an \textit{orchestration mechanism} is needed to manage the flow of messages between agents, to ensure that progress is made towards the completion of the task, and to handle the inevitable cases where an agent deviates from instructions. 
In this work we adopt this multi-agent paradigm, where agents are first-class citizens, acting as message transformers, and communicate by exchanging messages.

\paragraph{Tools}
%\textbf{Tools.}
As elucidated above, an LLM is essentially a text transformer; \ie in response to some input text (known as a \textit{prompt}), it produces a response. 
Free-form text responses are ideal when we want to generate a description, answer, or summary for human consumption, or even a question for another agent to answer. 
However, in some cases, we need the responses to trigger external \textit{actions}, such as a database query, web search, API call, or code execution. 
Then, we instruct the LLM response to be \textit{structured}, typically in JSON format, with various pre-specified fields, such as code, an SQL query, parameters of an API call, and so on. 
These structured responses have come to be known as tools, and the LLM is said to use a tool when it produces a structured response corresponding to a specific tool. 
To elicit a tool response from an LLM, it needs to be instructed on the expected tool format and the conditions under which it should use the tool.
Such tool-use capability allows LLM-based agents to leverage external tools and resources to accomplish tasks enhancing their functional capabilities, and operate more effectively in diverse and dynamic environments.

\paragraph{Memory}
%\textbf{Memory.}
In contrast to a solitary LLM, an agent maintains memory, which encompasses accumulated message history, detailing all queries and responses involving the agent, or external databases, facilitating in-context learning~\cite{brown2020language} to retain and retrieve information over prolonged periods. 
This capability enhances contextual coherence and fosters learning from interactions, crucial for navigating complex tasks efficiently.

As mentioned above, in constructing a system with multiple agents to tackle intricate tasks, an orchestration mechanism is critical to managing message flow between agents, ensuring task progression, and handling deviations from instructions. 
In our implementation, we build upon the Langroid library, which offers a simple yet versatile orchestration mechanism for agents, seamlessly managing user interaction, tool utilization, and sub-task delegation.


\input{figure_rag}

\subsection{Implementation Details}
\label{sec:ours-details}

% Drawing upon the external knowledge derived from the documents of all users, \ours tailors personalized responses to users' requests. 
% Our multi-agent RAG system comprises three pivotal agents: the Planner, Rule Manager, and Document Handler. 
% Below, we delineate the tasks, tools, and resources assigned to each agent.

Our framework first asks the users to write down their adaptation requests or rules into documents and then preprocesses them into a database (\textit{data ingestion}).
Referring to the personalized data, the three core agents in \ours collaborate with each other to support the three phases in MAP framework: reflection, articulation, and feedback.
The reflection stage is facilitated by the \textit{Rule Manager} and \textit{Document Handler} agents; Document Handler serves as the lowest-level agent that directly extracts structured information from the database, while the medium-level agent, Rule Manager ensures that Document Handler extracts all users' relevant information.
% , which analyze user information and extract structured data from documents. 
At the highest level, the \textit{Planner} agent initiates interaction with the user and incorporates the hierarchical orchestration with the Rule Manager and Document Handler.
It handles the articulation and feedback stages seamlessly; it generates personalized responses with the guidance of the Rule Manager, addresses conflicts that may arise in satisfying all users' preferences, and provides explanations for its responses upon request. 
% Through this orchestrated interaction among the agents, our system effectively supports the iterative process of reflection, articulation, and feedback, enabling adaptive personalization tailored to the needs of multiple users.
Below we describe the implementation details of the three agents, and tasks, tools, and resources assigned to each of them.
For an illustrative description of the overall process of \oursend, refer to Figure~\ref{fig:rag}.

%\textbf{Data Ingestion.~} 
\paragraph{Data Ingestion} At the onset of the interaction, users are asked to furnish their preferences in documents (depicted as step \redcircle{1} in Figure~\ref{fig:rag}).
These documents contain information pertinent to each user, encompassing individual requests, schedules, or rules. 
Subsequently, a pre-processing, or \textit{ingestion phase} ensues, wherein documents are sharded into reasonable-size chunks.
% and ingested into a suitable type of document store.
Each document chunk is mapped to a vector embedding via an embedding model (\eg BAAI/bge-large-en-v1.5~\cite{bge_embedding} in our implementation).
This process capitalizes on the inherent ability of vector embeddings to encapsulate the meaning of sentences or paragraphs~\cite{mikolov2013distributed, pennington2014glove, devlin2018bert}. 
Each vector embedding is then ingested into a vector database, along with a pointer to the chunk contents as metadata.

% Once done with the ingestion phase, Document Handler, one of the core building blocks of \ours, has access to the document store, and takes the role of retrieving chunks relevant to the query given to it, based on a notion of \textit{relevance} (details in Section~\ref{sec: ours-implementation}).

\iffalse
% During the query phase, the same embedding model is used to map the query into a vector, and then the top-$k$ nearest-neighbors of this vector (based on cosine similarity) are found from the vector database, and their corresponding document-chunks are retrieved.

% In the simplest case, the documents are short enough to comfortably fit within the LLM's context window (and still leave room for the question and answer). In this case, one could prompt the LLM in the form: ``Given the passages below: [passages] , answer this question: [question]'' One could refer to this simply as ``Augmented Generation'', since we are simply augmenting the user's query with the documents under consideration, and asking the LLM to generate an answer.

When the documents are long, however, one needs to use the RAG technique, which involves two phases: (1) a pre-processing or \textit{ingestion} phase where documents are sharded into reasonable-size chunks and ingested into a suitable type of document store (further details below), 
and (2) a query phase, where top-$k$ document-chunks most \textit{relevant} to the query are retrieved from the document store, and the LLM is prompted to answer the query given these chunks. The intuition here is that these relevant chunks will contain sufficient information for the LLM to be able to compose a reasonable answer.

Not surprisingly, the performance (\ie precision and recall of answers) of a RAG system depends critically on the ingestion and retrieval phases, and in particular on how we define what it means for a document-chunk to be ``relevant'' to a query. 

A number of retrieval techniques have emerged in the past year, and here we confine ourselves to an outline of the basic ideas. 
Broadly speaking there are two types of relevance: (1) \textit{lexical relevance}, which is the traditional notion of relevance based on word-overlap between the query and the document-chunk (\ie keyword search), and (2) \textit{semantic relevance}, which is a more flexible notion of relevance based on similarity of meaning between the query and the document-chunk. The most common way to determine semantic relevance is to leverage the fact that vector embeddings tend to encode meaning of sentences or paragraphs~\citep{mikolov2013distributed, pennington2014glove, devlin2018bert}: during the pre-processing phase, each document chunk is mapped to an embedding vector using an embedding model and this vector is indexed into a \textit{vector database}, along with a pointer to the chunk contents as metadata. 
During the query phase, the same embedding model is used to map the query into a vector, and then the top-$k$ nearest-neighbors of this vector (based on cosine similarity) are found from the vector database, and their corresponding document-chunks are retrieved. In a typical RAG system, a combination of lexical and semantic relevance is used to determine the top-$k$ most relevant chunks and this is what we do in this work.

\fi

% \subsubsection{\ours, a Specific instantiation of MAP Framework}
% \label{sec: ours-implementation}



\paragraph{Rule Manager}
The Rule Manager is tasked with extracting structured information from documents and presenting it in a specific nested format.
The JSON structure is explicitly defined for all users, where the highest-level fields represent users (\eg Blaine, Ryan, and Susie in Figure~\ref{fig:rag}).
Under each user field, the Rule Manager defines subfields to maximize information retrieval from the document.
Rule Manager generates questions corresponding to each field in the nested format and passes them, one by one, to the Document Handler (step \redcircle{5}) who has direct access to documents (more specifically, the vector database constructed from the ingestion phase).
% Rule Manager does not have access to documents, but it generates questions corresponding to each field in the JSON format, one by one, and pass it to Document Handler, who has direct access to documents (more specifically, the vector database constructed from the ingestion phase).
If the Document Handler cannot provide an answer to a question, the Rule Manager rephrases the question and retries a few more times until an answer is obtained. 
Once all fields in the structured format are filled, the Rule Manager returns the retrieved information to the Planner using a tool message (step \redcircle{9}).

\paragraph{Document Handler}
The Document Handler has direct access to documents and vector database, and is responsible for answering questions generated by the Rule Manager.
Given a question, this agent retrieves the top-$k$ most \textit{relevant} document-chunks from the vector database (step \redcircle{6} and \redcircle{7}).
It employs a combination of two notions of relevance: (a) \textit{lexical relevance}, so-called keyword search, which is based on word-overlap between the query and the document-chunk, and (b) \textit{semantic relevance}, which is a more flexible notion of relevance based on similarity of meaning between the query and the document-chunk. 
To determine semantic relevance, the question is mapped to a vector embedding using the same embedding model as in the ingestion phase, and the top-$k$ nearest-neighbors of this vector (based on cosine similarity) are found from the vector database, and their corresponding document-chunks are retrieved. 
The original question from Rule Manager is augmented with the retrieved document-chunks, and given the augmented question, Document Handler provides an answer to Rule Manager (step \redcircle{8}).

\paragraph{Planner}
The Planner serves as the highest-level interface between the system and the user. 
It is scheduled to talk to the Rule Manager first to reflect on user information (step \redcircle{3} and \redcircle{4}), then answer the user request.
By referring to the information returned by the Rule Manager (step \redcircle{9}), the Planner generates personalized responses to the user (step \smallerredcircle{10}).
These responses are tailored by considering all users' relevant information, and the Planner addresses any conflicts that may arise when satisfying all user's preferences. 
Additionally, the Planner articulates the reasoning behind its responses, providing a summary of relevant rules referred to, upon request.
These requirements are expressed in the Planner's system prompt as follows:
\noindent
\begin{Verbatim}[commandchars=\\\{\}, fontsize=\small]
    [...]
    MAKE SURE that NONE of your answers conflicts with ANY of the rules that you figured out in the first step.
    When assisting users, if ANY user has overlapping conflicts from their preferences and schedules 
    with another user, serve them in ALPHABETICAL ORDER of the users' names. 
    Once you present your answer, then I may ask for articulation of your response 
    with a summary of relevant rules that you referred to. 
    Then you should provide the explanation.
    [...]
\end{Verbatim}
The Planner maintains conversation history throughout interactions to keep track of the user's previous prompts and the corresponding responses, often followed by user feedback.

% Our system with these three agents can support the three core stages of MAP framework: reflection, articulation, and feedback; Reflection is done by Rule Manager and Document Handler. Articulation and Feedback are naturally handled by Planner.
% All put together, \ours, our proposed system with the three agents, is now ready to support




The source code for \ours implementation can be found in the anonymized repository.\footnote{The anonymized source code for \ours implementation can be found at \url{https://anonymous.4open.science/r/rag-for-multiuser-adaptive-personalization-F4F4}}
% We provide the anonymized codes for our implementation at: \href{https://anonymous.4open.science/r/rag-for-multiuser-adaptive-personalization-F4F4}{link to anonymous repository}.
% % \url{https://anonymous.4open.science/r/rag-for-multiuser-adaptive-personalization-F4F4}


==> workflow.tex <==
\section{Development of Multi-user Personalization Workflow}\label{sec:workflow}

This section outlines the development of the multi-user personalization workflow. 
We begin by defining the task, highlighting the key differences between single-user and multi-user personalization, with a focus on how the latter introduces the need to address and resolve conflicts (Section~\ref{sec:task}). 
Building on the distinctive challenges of multi-user tasks, we propose an expected workflow an AI system should follow to effectively support the multi-user personalization tasks, drawing on principles from conflict resolution literature (Section~\ref{sec:fw2}).
Finally, we present empirical evidence demonstrating that a basic LLM-based approach is not sufficient to achieve the desired workflow, thereby motivating our advanced approach based on the orchestration of multiple LLM-powered agents (Section~\ref{sec:motivation}).


%, we develop a workflow based on insights from conflict resolution literature, tailored to the specific demands of multi-user tasks.

% \subsection{Single-user vs Multi-user Personalization}
\subsection{Complexities in Multi-user Personalization}
\label{sec:task}
% \jihye{any references? \\}

\iffalse
The tasks and interaction requirements of human-AI interaction differ depending on whether the interaction involves a single user or multiple users.

In \textit{single-user} interactions, the interaction revolves around adapting the system to an individual's preferences and rules. The requirements in this setting are simpler, as the system only needs to account for one set of preferences, leading to a more straightforward decision-making process. The system's focus is on efficiently handling and personalizing tasks for the single user, ensuring that their unique needs are met without external conflicts.

On the other hand, \textit{multi-user} interactions introduce a more complex dynamic. The system must handle diverse, and often conflicting, preferences from multiple users. The requirements here extend beyond simple personalization, as the system must also identify and address potential conflicts between users' preferences and schedules. This creates a more intricate interaction dynamic, where resolving these conflicts and balancing competing needs becomes a central task, resulting in more layered requirements for the AI system.
\fi 

The tasks and interaction requirements for human-AI interactions differ significantly depending on whether the personalization task involves a single user or multiple users.

In \textit{single-user} interactions, the system focuses on adapting to the preferences and rules of an individual. This setting presents simpler requirements since the system only needs to consider one user's preferences, resulting in a straightforward decision-making process. The primary goal is to efficiently manage and personalize tasks to meet the unique needs of the individual without encountering external conflicts.

In contrast, \textit{multi-user} interactions introduce a more complex dynamic. The system must accommodate diverse and often conflicting preferences from multiple users. Requirements extend beyond basic personalization to include the identification and resolution of conflicts between users' preferences and schedules. This creates a more intricate interaction, where balancing competing needs and resolving conflicts become central tasks, leading to more sophisticated requirements for the AI system.


%\jihye{1) first define the target tasks: 1-1) the basic single-user personalization where the key focus is on adapting to user-specific preferences and rules, and 1-2) the multi-user personalization where the additional focus is addressing and resolving the conflicts between the users.2) }


 

% for multi-user conflict resolution and adaptive personalization. 
% In Section \ref{sec:fw1}, we discuss the details of the mutual's interaction workflow---reflection, articulation, and feedback. 


% \subsection{Framework Inspiration from Lifelong Learning Theory} \label{sec:fw1}


% We integrate this concept of lifelong learning into our framework designed for adapting AI systems to various personalization requirements from multiple end-users. This framework outlines a methodical approach to teaching AI systems to navigate constantly shifting user preferences and requests essential for personalization. The goal of this framework is to enable AI systems to understand \textit{how}, the adaptation process rather than the specifics of what to adapt. By learning how to adjust to the emerging needs of users or changes in the environment, AI systems can reflect on accumulated knowledge and diverse user preferences, demonstrate their learning application, and seek user or environmental feedback for further refinement or updates.



% \subsection{Interaction Stages: Reflection, Analysis, and Feedback}
\subsection{Proposed workflow: Reflection, Analysis, and Feedback}
\label{sec:fw2}

\iffalse
Given these increased complexities in multi-user settings, addressing conflicts and incorporating effective resolutions is crucial. 
We bring inspiration from conflict resolution literature and propose a workflow for multi-user personalization.

To support multi-user personalization in LLMs, we developed a workflow inspired by conflict resolution literature, aimed at guiding users when engaging with LLMs in multi-user settings.

Conflict resolution has been a long-standing research focus, ranging from interpersonal relationships to international disputes. Existing work highlights how conflict resolution seeks to understand the differing values of disputants and pave a path to resolution by merging and negotiating essential needs and interests \cite{thyagaraju2008conflict, rothman1997action}. In this area of research, \citet{ross2001action} presents an action-evaluation methodology that seamlessly integrates evaluation processes with conflict resolution. This approach focuses on achieving goals through resolution by following three stages: reflection, analysis, and feedback.
In the reflection stage, participants reflect on their motivation, values, and goals for the conflict resolution process. The analysis stage involves developing a working agenda or intervention plan to address these conflict resolution goals. Finally, the feedback stage revisits and revises goals, for continuous assessment of progress ad participants' satisfaction in conflict resolution.


Adopting this structure, we define three stages in our multi-user personalization workflow: reflection, analysis, and feedback. During the \textit{reflection} stage, the LLM gathers personalization elements from various users---such as preferences, interaction history, and schedules---to generate plans based on the users' requests. 
In the \textit{analysis} stage, the LLM constructs a plan based on collecting every users personalization elements. If conflict is detected among users for personalization, the LLM attempts to generate a resolution. Once the final multi-user personalization plan is complete, the LLM  presents and explains the results to users, outlining the decision-making process, rules considered, any conflicts detected, and resolutions for such conflicts. 
Finally, in the \textit{feedback} stage, the LLM incorporates user input on its performance. Feedback may include new preferences, adjustments to decision-making, or updates to existing settings. The LLM integrates this feedback to enable continuous refinement and better alignment with user needs.
\fi

Given the increased complexities in multi-user settings, it is crucial to adapt to personalized rules while effectively managing conflicts among users and incorporating resolution strategies. Specifically, we draw on conflict resolution literature and propose a workflow to guide AI systems in facilitating multi-user personalization.

Conflict resolution has been a longstanding area of research, ranging from interpersonal relationships to international disputes. Existing studies emphasize understanding the differing values of disputants and negotiating a path to resolution that satisfies essential needs and interests \cite{thyagaraju2008conflict, rothman1997action}.
In this area of research, \citet{ross2001action} introduces an action-evaluation methodology that integrates evaluation processes with conflict resolution. This approach includes three stages: reflection, analysis, and feedback.
In the reflection stage, participants reflect on their motivation, values, and goals for resolving the conflict. The analysis stage involves developing an intervention plan to achieve these goals. Finally, the feedback stage revisits and revises the goals for continuous assessment of progress and participants' satisfaction in conflict resolution.

Adopting this structure, we define a three-stage workflow for AI systems managing multi-user personalization:
\begin{enumerate}
    \item \textit{Reflection}: The AI system gathers personalization elements from various users, such as preferences, interaction history, and schedules.
    \item \textit{Analysis}: The AI system constructs a comprehensive plan by integrating each user's personalization elements. If conflicts arise, the LLM attempts to generate resolutions. Once a final multi-user personalization plan is formulated, the AI system presents and explains the outcomes to the users, detailing the decision-making process, the rules considered, detected conflicts, and the proposed resolutions.
    \item \textit{Feedback}: The AI system collects user feedback on its performance, which may include new preferences, adjustments to decision-making, or updates to existing settings. This feedback is then used to refine the system continuously, enhancing alignment with user needs.

\end{enumerate}



\input{figure_eval}
\subsection{Limitations of basic LLM-based approach for Multi-user Personalization}
\label{sec:motivation}

A natural question arises: can we simply use an LLM to construct the AI system for multi-user personalization? LLMs like GPT-4~\cite{gpt-4} are well known for their long-enough context window, advanced reasoning capabilities, and handling nuanced language—qualities that seem well-suited for complex personalization tasks. 
One might assume that a basic chat agent, wrapping an LLM with conversation history, could be sufficient to support the proposed workflow. In this subsection, we conduct a quantitative evaluation of the chat agent under three different personalization scenarios to assess its limitations.

% \subsubsection{Procedure}
\paragraph{Setup}
%The evaluation measures each model's success in accurately retrieving the rules and resolving the conflicts in each scenario.
Our evaluation considers personalization in three scenarios: (1) Automated Scheduling, where employees in a workplace have different meeting schedules and preferences for meeting environments; (2) Assistive Care with Robot, where residents in a care facility have distinct needs and schedules; and (3) Smart-Home Temperature Setting, where household members require different room temperatures based on their schedules (further details in Section~\ref{sec:scenarios}).
Each scenario involves 60 rules related to the preferences and schedules of three users, with 12 conflicts arising from overlapping preferences and schedules.
% For example, a scheduling conflict occurred when both Blaine and Ryan woke up at 7 am---Blaine requesting a greeting from the robot, along with a glass of water and her wheelchair prepared, while Ryan preferred three knocks on his door and for his shaving supplies to be placed on his bedside table. An overlapping preference conflict occurred with mail delivery: Blaine preferred her mail and packages delivered directly to her, whereas Susie preferred her mail to be left in a basket outside her door and packages delivered directly to her. If unavailable, Susie requested that packages be delivered to a human caretaker.

In Figure~\ref{fig:eval}, we interact with a basic chat agent with GPT-4 (denoted as ``LLM'' with the red bars) across these scenarios. Our evaluation focuses on two criteria: Retrieval (reflecting how well the system accounts for all user rules, a baseline requirement for any personalization) and Conflict Resolution (identifying conflicts among users and suggesting suitable resolutions, a key challenge in multi-user personalization). We measure (1) the percentage of the 60 rules correctly retrieved and incorporated into responses (``Retrieval''), and (2) the percentage of the 12 conflicts that were successfully identified and resolved (``Conflict'').


\paragraph{Limited effectiveness of single LLM-based chat agent.}
The results indicate that the basic LLM-based approach is insufficient for both Retrieval and Conflict Resolution functionalities. With a limited retrieval rate (~50\%) of user preferences and schedules, the system often fails to generate responses that fully account for all user rules, leading to inadequate conflict resolution (~30\% at the lowest). 
Specific errors included missing conflicts, failing to generate accurate plans for overlapping schedules (\eg multiple users requesting the same meeting room at 12:00 pm on Friday), or disregarding one user's preferences that negatively affected another (\eg one requesting the temperature never exceed 70\degree C, while the other wanted the home gym set to 80\degree C).

%integrating multiple users' preferences and schedules and resolving conflicts while creating multi-user personalized action plans.

%Each model was tested three times per the three scenarios described in \ref{sec:scenarios}. As one test outputs five daily action plans for the weekdays, we obtained 15 instances for each scenario, culminating in 45 instances for each condition, resulting in 90 instances in total for our validation. In each scenario, there were three users, each with 10 scheduling rules and 10 preference rules that the system was required to adhere to. We then compared each generated output against a reference solution provided by the researcher who formulated the scenarios. We measured the occurrence of errors, specifically where the models failed to correctly align with the intended schedules or preferences. The comparative results are shown in Figure \ref{fig:eval}. This analysis was conducted by two coders independently to minimize oversight. Although intercoder reliability was not collected, the coders iteratively discussed and refined their approach to identifying errors in the model outputs.

\paragraph{Motivating the multi-agent approach.}
These observations suggest the need for a more sophisticated mechanism that ensures complete awareness of all user rules and identifies and resolves conflicts effectively. As personalization complexity grows—with more users, rules, and nuances—a single, monolithic agent becomes increasingly inadequate. Moreover, imposing the proposed workflows for multi-user personalization (Section~\ref{sec:fw2}) onto a monolithic AI design proves challenging.
To address these issues, we propose a modular design in which the AI system operates through the orchestration of multiple specialized agents. Each agent is assigned specific subtasks and roles to collaboratively achieve the overall personalization goal. For example, one agent could focus on gathering user rules, monitored by another agent ensuring no rules are missed, thereby improving Retrieval accuracy. Another agent might be responsible for reasoning about potential conflicts, hence leading to enhanced Conflict Resolution.
Indeed, as shown by the blue bars labeled ``LAMP'' in Figure~\ref{fig:eval}, our multi-agent approach demonstrates significant improvements in both measures across all scenarios compared to the single LLM-based chat agent.

In the next section, we detail the implementation of LAMP, our multi-agent approach to multi-user personalization.

